The Highest Redshift Radio Galaxies

At low redshifts powerful radio sources are uniquely associated with massive galaxies, and are thought to be powered by supermassive black holes. Modern 8m -- 10m telescopes may be used used to find their likely progenitors at very high redshifts to study their formation and evolution.

==> report <==
%% report.bib - contains BiBtex input for bibliography

@book{Eisenberg92, 
	author = "A. Eisenberg", 
	title  = "Guide to Technical Editing", 
	publisher= "Oxford University", 
	address= "New York", 
	year   = "1992"	}

@book{Gelman95, 
	author = "A. Gelman and J. B. Carlin and H. S. Stern and D. B. Rubin", 
	title  = "Bayesian Data Analysis", 
	publisher= "Chapman \& Hall", 
	address= "London", 
	year   = "1995"	} 

@incollection{Gull89a, 
	author = "S. F. Gull", 
	title  = "Developments in maximum-entropy data analysis", 
	booktitle= " Maximum Entropy and Bayesian Methods", 
	editor = "J. Skilling", 
	pages  = "53-71 ", 
	publisher= "Kluwer Academic, Dordrecht", 
	year   = "1989"	} 
 
@inproceedings{Hanson93c, 
	author = "K. M. Hanson", 
	title  = "Introduction to {B}ayesian image analysis", 
	booktitle= "Image Processing",
	editor = "M.\ H. Loew",
	journal= "Proc. SPIE", 
	volume = "1898",
	pages  = "716-731", 
	year   = "1993"	} 

@book{Lamport94, 
	author = "L. Lamport", 
	title  = "LaTeX: A Document Preparation System", 
	publisher= "Addison-Wesley", 
	address= "Reading", 
	year   = "1994"	}

@article{Metropolis53, 
	author = "N. Metropolis and A. W. Rosenbluth and M. N. Rosenbluth and A. H. Teller and E. Teller", 
	title  = "Equations of state calculations by fast computing machine", 
	journal= "J. Chem. Phys.",  
	volume = "21", 
	pages  = "1087-1091", 
	year   = "1953"	} 
 

 



